TextSphere: Efficient Text-to-Image Generation via Shared Hyperspherical Alignment and Uniformity

Recent advances in text-to-image generation have substantially improved image quality, particularly through diffusion-based methods that require multiple inference steps. In contrast, Sphere Encoder offers an efficient generative framework capable of producing images with fewer forward steps. However, extending it to free-form text is nontrivial, because its class-conditioned design lacks cross-modal alignment. To address this challenge, we propose TextSphere, an efficient text-to-image generative framework that extends Sphere Encoder with language conditioning and cross-modal alignment. We incorporate pretrained CLIP text embeddings through adaptive layer normalization (AdaLN) to guide image generation while retaining the original spherical sampling mechanism. To bridge the cross-modal representation gap, we introduce a Spherical Semantic Alignment and Uniformity (SSAU) objective that jointly promotes semantic alignment and representation uniformity on the hypersphere. Experiments on CUB-200-2011, MS-COCO-2014, and Flickr30k demonstrate that TextSphere consistently reduces generation FID (gFID) over the text-conditioned baseline while achieving reconstruction FID (rFID) below 1.0. With only 4 and 6 sampling steps, TextSphere achieves lower gFID than the compared diffusion- and GAN-based models trained from scratch on CUB-200-2011 and MS-COCO-2014, respectively. We further observe that improved reconstruction fidelity does not necessarily yield better generation quality. In addition, we use Partial Least Squares Singular Value Decomposition (PLS-SVD) to analyze cross-modal alignment and modality gap, offering insight into the effectiveness of our approach.

==> Fig/teaser.tex <==
\begin{strip}
\centering
\includegraphics[width=.33\linewidth]{example-image-golden}\hfill
\includegraphics[width=.33\linewidth]{example-image-golden}\hfill
\includegraphics[width=.33\linewidth]{example-image-golden}
\captionsetup{hypcap=false}
\captionof{figure}{\textbf{Teaser} -- example of a 2-column teaser. This figure appears at the top of the first page, and a two-column teaser is not mandatory.}
\captionsetup{hypcap=true}
\label{fig:\currfilebase}%
\end{strip}
